SpiderCSS: Scalable Fault-Tolerant CSS State Preparation

Fault-tolerant preparation of logical states is a critical primitive for the realization of large-scale fault-tolerant quantum computing. This paper introduces SpiderCSS, a scalable compilation pipeline that generates highly-optimized, fault-tolerant state preparation circuits for arbitrary Calderbank-Shor-Steane (CSS) codes. Starting from an idealized specification of a CSS state, we use the ZX-calculus and fault-equivalent rewrites to construct a diagram that prepares the given state while preserving the fault tolerance of the initial ideal ZX-diagram. From this diagram, SpiderCSS constructs a fault-tolerant CSS-state preparation circuit using a modular construction that is CNOT-minimal both within each component and also in the way these components are connected together. By only using fault-equivalent rewrites, the final circuit is provably fault-tolerant without needing expensive verification. Monte Carlo simulations across a variety of CSS codes up to distance 15 show that SpiderCSS scales efficiently and constructs circuits with substantially reduced depth and qubit footprint compared to existing scalable and heuristic methods, while simultaneously achieving an average decrease of 33.7% in logical error rate and an increase of 9.5% in acceptance rate.

==> extraction_example_figure.tex <==
\begin{figure*}[htp]
  \centering
  \begin{subfigure}[b]{0.50\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/steane_forest}
    \caption{The global graph $G_{\text{global}}$ with the spanning forest $F_{\text{global}}$ marked with blue edges. Nodes marked with red circles correspond to $X$ spiders while green circles correspond to $Z$ spiders. Bipartite edges are marked yellow.}
    \label{fig:steane_forest}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/steane_digraph}
    \caption{The global dependency directed acyclic graph $D_{\text{global}}$. Yellow edges correspond to CNOT gates. Red edges correspond to artificial insertions of CNOT orderings according to \Cref{subsec:well-ordered-cat-states}.}
    \label{fig:steane_digraph}
  \end{subfigure}
  
  \vspace{0.5em}
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/steane_circuit}
    \caption{The final extracted fault-tolerant circuit, ticks are inserted after processing each topological generation of $D$.}
    \label{fig:steane_circuit}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \begin{minipage}[t]{0.48\textwidth}
{\fontsize{6.5}{7.5}\selectfont
\begin{verbatim}
Init Root 0 (Tree 0) -> Q0
Init Root 5 (Tree 1) -> Q1
Init Root 9 (Tree 2) -> Q2
Init Root 14 (Tree 3) -> Q3
Init Root 18 (Tree 4) -> Q4
Init Root 23 (Tree 5) -> Q5
Init Root 27 (Tree 6) -> Q6
Node 0 -> Branch 2: Spawned CNOT Q0 -> Q7
Node 0 -> Primary 1 (Inherits Q0)
Node 5 -> Primary 6 (Inherits Q1)
Node 9 -> Branch 11: Spawned CNOT Q2 -> Q8
Node 9 -> Primary 10 (Inherits Q2)
Node 14 -> Primary 15 (Inherits Q3)
Node 18 -> Branch 20: Spawned CNOT Q4 -> Q9
Node 18 -> Primary 19 (Inherits Q4)
Node 23 -> Primary 24 (Inherits Q5)
Node 27 -> Branch 29: Spawned CNOT Q6 -> Q10
Node 27 -> Primary 28 (Inherits Q6)
Adding CNOT at (1, 6): CNOT Q0 -> Q1
Node 6 -> Primary 7 (Inherits Q1)
Skipping CNOT edge at (1, 6)
Node 1 -> Primary 3 (Inherits Q0)
Adding CNOT at (2, 15): CNOT Q7 -> Q3
Node 15 -> Primary 16 (Inherits Q3)
Skipping CNOT edge at (2, 15)
Node 2 -> Primary 4 (Inherits Q7)
Adding CNOT at (20, 24): CNOT Q9 -> Q5
Node 24 -> Primary 25 (Inherits Q5)
Skipping CNOT edge at (20, 24)
Node 20 -> Primary 22 (Inherits Q9)
Adding CNOT at (7, 19): CNOT Q4 -> Q1
Node 7 -> Primary 8 (Inherits Q1)
Skipping CNOT edge at (7, 19)
\end{verbatim}
}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\textwidth}
{\fontsize{6.5}{7.5}\selectfont
\begin{verbatim}
Node 19 -> Primary 21 (Inherits Q4)
Adding CNOT at (16, 28): CNOT Q6 -> Q3
Node 16 -> Primary 17 (Inherits Q3)
Skipping CNOT edge at (16, 28)
Node 28 -> Primary 30 (Inherits Q6)
Node 4 assumes the role of a flag qubit for edge (3, 4) on Q7.
Adding CNOT at (4, 10): CNOT Q7 -> Q2
Skipping CNOT edge at (4, 10)
Node 10 -> Primary 12 (Inherits Q2)
Adding CNOT at (25, 29): CNOT Q10 -> Q5
Node 25 -> Primary 26 (Inherits Q5)
Skipping CNOT edge at (25, 29)
Node 29 -> Primary 31 (Inherits Q10)
Node 22 assumes the role of a flag qubit for edge (21, 22) on Q9.
Adding CNOT at (11, 22): CNOT Q9 -> Q8
Skipping CNOT edge at (11, 22)
Node 11 -> Primary 13 (Inherits Q8)
Node 8 serves as a sink point for Q1
Node 17 serves as a sink point for Q3
Flag (3, 4) finalised: CNOT Q0 -> Q7; PostSelect_Z 7
Node 3 serves as a sink point for Q0
Node 26 serves as a sink point for Q5
Flag (21, 22) finalised: CNOT Q4 -> Q9; PostSelect_Z 9
Node 21 serves as a sink point for Q4
Node 13 assumes the role of a flag qubit for edge (12, 13) on Q8.
Adding CNOT at (13, 31): CNOT Q10 -> Q8
Node 31 assumes the role of a flag qubit for edge (30, 31) on Q10.
Skipping CNOT edge at (13, 31)
Flag (12, 13) finalised: CNOT Q8 -> Q2; PostSelect_X 8
Node 12 serves as a sink point for Q2
Flag (30, 31) finalised: CNOT Q6 -> Q10; PostSelect_Z 10
Node 30 serves as a sink point for Q6
\end{verbatim}
}
\end{minipage}
    \caption{The raw log of the circuit extraction procedure indicating the graph traversal order and the corresponding operations.}
    \label{fig:log}
  \end{subfigure}


  \caption{Example circuit extraction for the Steane code.}
  \label{fig:steane_appendix_example}
\end{figure*}

